Predictive Inequity in Object Detection

In this work, we investigate whether state-of-the-art object detection systems have equitable predictive performance on pedestrians with different skin tones. This work is motivated by many recent examples of ML and vision systems displaying higher error rates for certain demographic groups than others. We annotate an existing large scale dataset which contains pedestrians, BDD100K, with Fitzpatrick skin tones in ranges [1-3] or [4-6]. We then provide an in-depth comparative analysis of performance between these two skin tone groupings, finding that neither time of day nor occlusion explain this behavior, suggesting this disparity is not merely the result of pedestrians in the 4-6 range appearing in more difficult scenes for detection. We investigate to what extent time of day, occlusion, and reweighting the supervised loss during training affect this predictive bias.

==> sources.tex <==

\iffalse \section{Disambiguating sources of predictive inequity}

In this section, we describe in detail three possible sources of inequitable predictive performance, focusing on  object detection's ability to identify pedestrians, and the experiments we designed to measure them. Unless we specify otherwise, any use of the word ``loss" refers to test loss. 

\iffalse


\jmcomment{all of these should probably have error bars around them...}

\jmcomment{These might be questions about training + data + model, not just data + model.}\fi

\subsection{Potential Source \#1: Optimization Imbalance}
The first hypothesis we investigate is to what extent the predictive inequity of pedestrian detection systems stems from emphasizing the accuracy or loss  for larger populations during model training.  Many loss functions place equal emphasis on each training example, naturally leading to a larger population having higher importance when minimizing loss. Simply considering reweightings of the (per-sample) loss terms will bias the selection process towards models with lower loss on higher weight samples. 

Reweighting has been proposed as a method for improving datasets and resulting models which fail to satisfy statistical parity~\citep{preprocessing} or equality of false positives and negatives~\citep{csc}. Here, we encourage reweighting as a method for measuring how much  predicitive inequity stems from inequity in importance during optimization. When this amount is large, reweighting will effectively reduce predictive inequity.

\iffalse

We now outline a straightforward test for optimization imbalance of a particular model and training algorithm. Suppose a training dataset $X$ has a $p \ll \frac{1}{2}$ fraction of data points from group $B$ and $1-p$ fraction from group $A$.
Produce a new optimization procedure such that $A$ and $B$  have equal importance in the objective value\footnote{One could (a)
 subsample points from $A$ or duplicate points in $B$ to produce a new dataset $X'$ with roughly equal proportions of points from $A$ and $B$ or (b) reweight the terms in the objective function.}. Then, run the training algorithm on $X'$, and measure the disparity in validation MAP on groups $A$ and $B$. We define the {\bf optimization imbalance} of this model class on this task to be the difference in this disparity from training on $X$ to $X'$.
 \fi

The important point about testing optimization imbalance is that reweighting \emph{should not}
 increase the amount of statistical power an algorithm has to generalize on the smaller population (in fact, it might decrease it). Reweighting instead should bias the algorithm toward producing models with lower error on higher-weight examples. 
 
 \paragraph{Evidence of Optimization Imbalance}
 
\iffalse \jmcomment{Should we say whether we look at train v test error? The goal of optimization in ML is to reduce test error, but that's almost always done by some constrained minimization of training error. Not clear which we should measure. I'll think about this more.}
 \jmcomment{I think we should look at test error. But I'll think about this a bit more.}
\fi


\subsection{Potential Source \#2: Measurement mismatch between images and these models}

Our second hypothesis is that the problem of detecting pedestrians with different skin tones might be fundamentally more difficult (a) for the algorithms we tend to use to train these models, (b) for this class of models on these images, or (c) that information-theoretically, the task of detecting  pedestrians in images from BDD100k is fundamentally harder when the pedestrians have darker skin tones. 


\newcommand{\A}{\mathcal{A}}
\newcommand{\M}{\mathcal{M}}
\newcommand{\E}{\mathbb{E}}
\newcommand{\pmi} {\textrm{PMI}}
\newcommand{\pmih} {\overhat{\textrm{PMI}}}

These three issues are not equivalent; the first refers to our computational ability to minimize loss for the two groups; the second to our choice of model class; and the third to a question of the information-theoretic difficulty of detection for pedestrians with differing skin tones. 
We present these concerns together rather than separately because they may be difficult or impossible to disentangle in real-world settings with computational and data constraints, where finding the best model can be computationally intractable and testing arbitrary other model classes will invariably lead to overfitting. So, for settings where the set of images and computational time are finite, we define the \emph{practical measurement imbalance in test} for loss $\ell$, for an algorithm $\A$ optimizing over model class $\M$, and samples $S,S'$ of size $n$ drawn from  distributions $D, D'$ from populations $X,X'$, to be 

\[\pmi_n = |\E_{S\sim D} [\ell(\A(S))] - \E_{S' \sim D'} [\ell(\A(S'))]|.\]

This quantity measures how well this particular algorithm does at optimizing $\ell$ for the sample from $D$ versus that from $D'$. It tacitly depends on the set of models the algorithm selects amongst, and does not differentiate between issues of computation and information. If the algorithm does poorly optimizing for a group, for practical purposes this is equivalent to the model class doing a poorer job for that group if this is the algorithm used to optimize over this class of models.

\begin{remark}
 We assume that the training datasets from the two different populations have equal size, to disambiguate the improvement $\A$ achieves from having a larger dataset for one population than the other.
\end{remark}

Of course, we cannot know exactly the expected loss of $A()$ on $D$, but instead only know some sampled estimate. If $A$ is trying to optimize $\ell$ (or something with positive correlation with $\ell$), one would expect that the training estimate $\pmih$
(which we call the \emph{practical measurement imbalance in train}), 
would only be smaller than \pmi.\footnote{\jmcomment{Do you guys understand why this is likely to be the case? I'm thinking decreasing marginal returns on optimizing things with lower loss, along with the fact that empirical loss is usually overly optimistic compared to true loss, and so it'll be more optimistic (I'd guess) for the larger loss...}}
It is also natural to assess the \emph{practical measurement imbalance in val}, which should be less biased than the training estimate. 

\paragraph{Potential Source \#3: Differing Statistical Significance}

The final hypothesis we test is the extent to which the training of object detection models is similarly generalizeable for different demographic groups of pedestrians. This idea that we will have higher statistical certainty about our predictions for larger populations is not new---this is likely what most people mean when they state that imbalanced predictive performance comes from too little data about smaller demographic groups. This intuition has several natural mathematical formulations: the simplest comes from arguing about the uniform convergence rates over the class $C$ of models used for the population size, given by standard VC-type bounds. 

Two natural classes measurements of differing statistical significance arise: those based on empirical measurements of generalization and those based on theoretical guarantees of the algorithms or models used. Most standard theoretical guarantees will show that, on a training dataset of size $m$ of both populations, where a $p> \frac{1}{2}$ fraction comes from population $A$ and a $1-p$ fraction comes from $B$, the confidence about the loss on $A$ will scale like $\frac{c}{\sqrt{mp}}$ and for $B$ like $\frac{c}{\sqrt{m(1-p)}}$, for $c$ dependent on the coverage probability and complexity of the model class or algorithm used to optimize. Either way, the amount that the smaller population's uncertainty can be blamed for poor performance on $B$ should not be larger than the confidence interval, namely $\frac{c}{\sqrt{m(1-p)}}$. 

In practice, and in the case of object detection, models used rarely have nice VC-dimension upper bounds, nor are there obvious arguments about whether the algorithms used to optimize over them should give strong generalization. Some basic understanding of why deep nets generalize make come from limiting their training iterations~\citep{}, but most of how we see these models perform in practice cannot be explained by current generalizeability theory~\citep{moritznn}. For this reason, we suggest that one measures the empirical amount of overfitting which occurs for $A$ versus $B$ (comparing train versus test, or train versus validation). So, fixing the training data, train a model $\M$ and measure the train versus test performance on examples from $A$ versus $B$; the change in train to test for $B$ is some measure of how poorly the model generalizes on examples from $B$.





\iffalse
Given that the training dataset has many more points from category $A$ than $B$, standard generalization arguments (such as arguing using a Chernoff bound) suggest that any fixed model's behavior in test would be closer to the model's behavior in train on group $A$ than $B$. So, even if there was no optimization imbalance, the variance of the learned model might be higher for $B$ than $A$, which might lead to worse performance for $B$ in test.


This bound may be overly pessimistic for a particular data distribution and hypothesis class,  thereby overestimating the amount of statistical uncertainty we might have about our predictions for the smaller population. Moreover, some evidence  suggests neural networks' generalizeability is very poorly characterized by such arguments\citep{moritznn}.

For this reason, we describe the difference in statistical significance a model displays for two different populations in a way that is flexible enough to argue both about hypothesis classes with low dimensionality (VC or otherwise), but also applies to settings without meaningful bounds on such a measure. Suppose a model $f$ is equipped with confidence intervals around its estimated loss for populations $A$ and $B$, respectively. Then, the degree to which the statistical uncertainty could lead to differing loss on $A$ versus $B$ is upper-bounded by the sum of the widths of those confidence intervals. All of the uncertainty about the model's predictions on $A$ versus $B$ is nicely captured in such a sum, regardless of the source of the confidence intervals (providing they accurately capture the intended uncertainty of the model's behavior with probability $1-\delta$). These confidence intervals can come from standard VC theory (for simpler model classes), centered around the empirical loss $f$ suffers for $A$ and $B$, or from the width of some hold-out estimates' confidence interval (the width of such a confidence interval will be $\sqrt{\frac{\ln\frac{2}{\delta}}{m_{hold}}}$, where $m_{hold}$
is the size of the holdout set). 

More formally, fix some confidence widths around some empirical estimate of $f$'s loss on $A$ and $B$ which hold with probability $1-\delta$, denoted $c_{A,\delta}, c_{B,\delta}$. Then, $c_{A, \delta}+c_{B, \delta}$ upper bounds the amount by which the uncertainty about $A$ or $B$ is responsible for differences in $f$'s loss for $A$ versus $B$. $c_{A,\delta}+c_{B,\delta}$ simply represents an upper bound on the uncertainty in $f$'s loss on $A$ and $B$.
\fi

\iffalse
\newcommand{\F}{\mathcal{F}}
\begin{definition}[Uniform Algorithmic Uncertainty]
Fix some loss functions $\ell_1, \ell_2$. 
Suppose an algorithm always ouptus a model from a class $\F$, and produces confidence widths $c_1, c_2$ such that, with probability $1-\delta$ for all $f\in\F$
\[ |\ell_1(f) - \hat{\ell_1}(f)| \leq c_1 \quad \textrm{ and } \quad|\ell_2(f) - \hat{\ell_2}(f)| \leq c_2 . \]
Then these confidence widths are said to hold uniformly over $\F$.\iffalse and upper bound the extent to which the algorithm's uncertainty about $\ell_1,\ell_2$ affects the value of those losses in optimization.
\end{definition}

This form of uncertainty, the uncertainty an algorithm has about the true $\ell_1,$ and $\ell_2$  loss of each model in its class, upper bounds the amount by which empirical estimates of said losses might be wrong as the algorithm selects amongst models from $\F$. Such an upper bound on the error of these empirical estimators also serves as a measurement of how much the uncertainty about $\ell_1,\ell_2$ can attribute to imbalance between $\ell_1,\ell_2$ observed in test.

For many models, and neural networks in particular, it can be difficult to bound the uniform uncertainty of a training algorithm. 

\begin{definition}[ uncertainty]

\end{definition}
\begin{remark}
These confidence intervals 
\end{remark}


\begin{enumerate}
    \item Vc theory tells us... not much interesting. something like the hold-out multiplied by $VC(d)$.
%    \item description length
    \item A simple hold-out set calculation (e.g., 11.1 in the understanding ML book). This would mean we'd get something like $\sqrt{\frac{\ln \frac{2}{\delta}}{m_A}} - \sqrt{\frac{\ln \frac{2}{\delta}}{m_B}}$. I think for the test set sizes we have, this'd be like $.0850$, which certainly could explain some fraction of the difference...
    \item some kind of $k$-fold cross-validation or other empirical measure of variance.
\end{enumerate}

To measure the imbalance in statistical significance of a method, we do the following. We compute the train and test MAP for both categories $A$ and $B$. Then, define the imbalance in statistical significance to be 
\[|\map_{test, B} - \map_{train, B} | - |\map_{test, A} - \map_{train, A} |. \]

This is simply comparing the variance of the \map of our algorithm broken down by group, using empirical estimators.



For a particular representation of driving environment and a particular model class $C$ and two types of object $X, X'$ draw from distributions $D, D'$ to predict, the best model to predict the first class might have better accuracy than the best model to predict the second. We refer to this as \emph{class-specific measurement imbalance}, and formally define it to be
\[\max_{f\in C} \map_{ D}(f) - \max_{f'\in C}\map_{ D'}(f') . \]
\bwcomment{We should probably decide on how we want to symbolically show "average precision". They've made it super confusing because some people say mAP to refer to the average of average precisions across classes, but MS COCO (via their website) refers to AP$_{50}$ being the average over all categories at 50\% IoU.}
\jmcomment{Ok makes sense. I'm using \map for now, which we can toggle as we like.}
That is, we measure how well any model can detect those objects in $X$ versus any model to detect those in $X'$.

Given that we do not have direct access to the true distributions $D,D'$, we measure an empirical estimate of this, by training a model for the training data with type A pedestrians and another one for data with type B pedestrians. This means we will train a model to detect class $A$ pedestrians from the training data, and a separate model to detect class $B$ pedestrians from the training data, and compare their MAP.
During training, we do not want to penalize ``false positives" that identify pedestrians of the opposite type. So, we  simply give those pedestrians $0$ weight in the objective function. 

\jmcomment{The size of the samples we train on should be the same.} \bwcomment{So I guess just $\min(|A_{training}|, |B_{training}|) = 789$?}

\paragraph{Set of Experiments to do for this source}


We want to both consider changing the training data and changing the objective function. In terms of changing the loss function, consider a loss function only containing terms:
\begin{itemize}
\item for Cat B (Particularly interesting, could be an ``augmenting net")
\item for Cat B / small   (somewhat interesting)
\item for Cat A/B / small 
\item for Cat B/non-people 
\item for Cat B/small/non-people (Also particularly interesting, in that we're doing an otherwise identical task but not caring about classifying category A)
\item for Cat A/B / small/ non-people (Original experiment)
\end{itemize}

The same could be done for training data, and  I think the interesting ones are the one whose only images are category B, category B and small people, category B and small people and non-people. \jmcomment{We could do these with or without loss function modification, I think it makes sense to first try without.}\fi
\fi

==> tables/BDDval_BDDtrain_no_occluded_compare-weightings.tex <==
\begin{table}
    \begin{center}
    \resizebox{\linewidth}{!}{
    \begin{tabular}{l  cc c cc c cc}
    	\toprule
    	  \multirow{2}{*}{\textbf{Model}}   & \multicolumn{2}{c}{\textbf{AP}}       && \multicolumn{2}{c}{\textbf{AP$_{50}$}} && \multicolumn{2}{c}{\textbf{AP$_{75}$}}\\
    	  \cmidrule{2-3}\cmidrule{5-6}\cmidrule{8-9}
    	  & A & B && A & B && A & B \\
    \hline
        \textbf{Unweighted}               & \textbf{0.550}  & 0.538          && 0.841          & \textbf{0.875} && \textbf{0.620}  & 0.598          \\
        \textbf{5x Weight on Category B}  & \textbf{0.589} & 0.561          && \textbf{0.882} & 0.862         && 0.691          & \textbf{0.707} \\
        \textbf{10x Weight on Category B} & 0.579          & \textbf{0.582} && 0.868          & \textbf{0.875} && \textbf{0.701} & 0.674          \\
        \hline
        \textbf{Average}                 & \textbf{0.573} & 0.560           && 0.864          & \textbf{0.871} && \textbf{0.671} & 0.660           \\
    \hline
    \end{tabular}
    }
    \end{center}
    \caption{Average precision on BDD100K validation set using Faster-RCNN with R-50-FPN backbone trained on BDD100K train set with occluded individuals removed using different weighting schemes.}
    \label{tab:bddval_no_occluded_compare-weighting}
    
\end{table}

==> turker-labelers.tex <==
We give the numeric representation of Figure~\ref{fig:hist_anno} in the table below.
\begin{table}
\begin{tabular}{ll}
\textbf{Label Sequence}        & \textbf{Count}    \\
LLL                            & 1921              \\
LLD                            & 416               \\
LLU                            & 373               \\
LLN                            & 14                \\
DDD                            & 400               \\
DDL                            & 232               \\
DDU                            & 153               \\
DDN                            & 4                 \\
Ignored for disparity analysis & \jmcomment{4979- Total above}
\end{tabular}
\caption{Breakdown of 3xlabel frequency}\label{table:turk}
\end{table}
